MPGE: A Multi-Perspective Graph Explainer for Molecular Classification Explanation

Graph neural networks (GNNs) predict molecular properties from chemical graph data, but predictive accuracy does not explain how graph information supports an individual decision. A compact prediction-preserving rationale does not necessarily reveal which changes reverse the decision or which modifications the model tolerates. We propose the Multi-Perspective Graph Explainer (MPGE), unifying factual support, counterfactual sensitivity, and exemplar tolerance for a frozen classifier. The factual view, originally termed prototype (PT), seeks a compact retained edge set with the same label and required confidence. Counterfactual (CF) explanations seek bounded prediction-changing deletions; exemplar (EXE) explanations seek non-trivial bounded deletions that preserve the label and confidence. A shared constrained formulation connects prediction behavior, compactness, and edit cost, while separate objectives generate the three views. Our graph-classification extension of CF-GNNExplainer learns symmetric edge rankings and verifies discrete candidates, recording unsuccessful searches. A separate BBBP fragment backend returns RDKit-sanitized molecules. We evaluate the primary GCN implementation on MUTAG, Mutagenicity, AIDS, COX2_MD, and BBBP using semantic coverage, conditional quality, stability, and runtime. Successful factual masks retained 8.6%--15.5% of input edges on average across datasets; bounded counterfactual coverage was 4.8%--67.6%, and exemplar preservation coverage was 98.9%--100.0%. Exploratory controls reveal the influence of hard projection and retained node information. Quantitative comparisons and molecular visualizations characterize model support, sensitivity, and tolerance without treating them as validated chemical mechanisms.

==> submission_all_dataset_explanations.tex <==
\begin{tabular}{lccc|ccc|ccc}
\toprule
& \multicolumn{3}{c|}{Factual} & \multicolumn{3}{c|}{Counterfactual} & \multicolumn{3}{c}{Exemplar} \\
Dataset & Success & Retained & Comp. & Success & Edits & $\Delta p_y$ & Success & Edited & Retained $p_y$ ratio \\
\midrule
MUTAG & 100.0\% & $0.105 \pm 0.131$ & $0.120 \pm 0.220$ & 67.6\% & $2.59 \pm 1.57$ & $0.436 \pm 0.192$ & 98.9\% & $0.279 \pm 0.048$ & $1.041 \pm 0.161$ \\
Mutagenicity & 100.0\% & $0.155 \pm 0.203$ & $0.142 \pm 0.241$ & 63.7\% & $2.85 \pm 1.91$ & $0.315 \pm 0.155$ & 99.0\% & $0.246 \pm 0.068$ & $1.046 \pm 0.129$ \\
AIDS & 100.0\% & $0.103 \pm 0.079$ & $0.019 \pm 0.113$ & 4.8\% & $3.48 \pm 2.10$ & $0.419 \pm 0.165$ & 100.0\% & $0.285 \pm 0.059$ & $1.002 \pm 0.040$ \\
COX2\_MD & 100.0\% & $0.092 \pm 0.218$ & $0.048 \pm 0.173$ & 5.5\% & $4.68 \pm 2.33$ & $0.099 \pm 0.114$ & 100.0\% & $0.025 \pm 0.005$ & $0.998 \pm 0.028$ \\
BBBP & 100.0\% & $0.086 \pm 0.093$ & $0.090 \pm 0.163$ & 54.6\% & $3.65 \pm 2.24$ & $0.382 \pm 0.146$ & 99.7\% & $0.277 \pm 0.052$ & $1.008 \pm 0.094$ \\
\bottomrule
\end{tabular}


==> submission_baseline_counterfactual.tex <==
\begin{tabular}{lllcc}
\toprule
Dataset & Method & Success & Edits & $\Delta p_y$ \\
\midrule
MUTAG & MPGX-CF & 67.6\% & $2.594 \pm 1.569$ & $0.436 \pm 0.192$ \\
MUTAG & CF-GNNExplainer & 3.7\% & $1.190 \pm 0.402$ & $0.398 \pm 0.118$ \\
MUTAG & CF$^2$ reimplementation & 7.2\% & $5.854 \pm 1.663$ & $0.756 \pm 0.202$ \\
MUTAG & Random & 31.3\% & $3.452 \pm 1.910$ & $0.396 \pm 0.187$ \\
\addlinespace
Mutagenicity & MPGX-CF & 63.7\% & $2.851 \pm 1.912$ & $0.315 \pm 0.155$ \\
Mutagenicity & CF-GNNExplainer & 2.2\% & $1.286 \pm 0.590$ & $0.335 \pm 0.127$ \\
Mutagenicity & CF$^2$ reimplementation & 1.3\% & $5.281 \pm 2.098$ & $0.321 \pm 0.209$ \\
Mutagenicity & Random & 22.5\% & $3.568 \pm 1.937$ & $0.231 \pm 0.140$ \\
\addlinespace
AIDS & MPGX-CF & 4.8\% & $3.475 \pm 2.100$ & $0.419 \pm 0.165$ \\
AIDS & CF-GNNExplainer & 0.1\% & $1.000 \pm 0.000$ & $0.380 \pm 0.090$ \\
AIDS & CF$^2$ reimplementation & 0.2\% & $4.300 \pm 1.925$ & $0.408 \pm 0.268$ \\
AIDS & Random & 1.2\% & $3.628 \pm 2.146$ & $0.330 \pm 0.173$ \\
\addlinespace
COX2\_MD & MPGX-CF & 5.5\% & $4.679 \pm 2.328$ & $0.099 \pm 0.114$ \\
COX2\_MD & CF-GNNExplainer & 0.0\% & -- & -- \\
COX2\_MD & CF$^2$ reimplementation & 0.3\% & $6.667 \pm 0.471$ & $0.041 \pm 0.052$ \\
COX2\_MD & Random & 1.0\% & $5.678 \pm 1.934$ & $0.060 \pm 0.059$ \\
\addlinespace
BBBP & MPGX-CF & 54.6\% & $3.647 \pm 2.244$ & $0.382 \pm 0.146$ \\
BBBP & CF-GNNExplainer & 0.2\% & $1.000 \pm 0.000$ & $0.369 \pm 0.000$ \\
BBBP & CF$^2$ reimplementation & 0.5\% & $6.250 \pm 1.255$ & $0.466 \pm 0.242$ \\
BBBP & Random & 10.6\% & $3.951 \pm 2.054$ & $0.238 \pm 0.131$ \\
\addlinespace
\bottomrule
\end{tabular}


==> submission_baseline_exemplar.tex <==
\begin{tabular}{lllcc}
\toprule
Dataset & Method & Success & Edited & Retained $p_y$ ratio \\
\midrule
MUTAG & MPGX-CF & 98.9\% & $0.279 \pm 0.048$ & $1.041 \pm 0.161$ \\
MUTAG & Greedy control & 100.0\% & $0.305 \pm 0.026$ & $1.169 \pm 0.232$ \\
MUTAG & Random & 94.6\% & $0.268 \pm 0.060$ & $1.023 \pm 0.145$ \\
\addlinespace
Mutagenicity & MPGX-CF & 99.0\% & $0.246 \pm 0.068$ & $1.046 \pm 0.129$ \\
Mutagenicity & Greedy control & 99.9\% & $0.257 \pm 0.069$ & $1.191 \pm 0.211$ \\
Mutagenicity & Random & 96.5\% & $0.231 \pm 0.074$ & $1.027 \pm 0.127$ \\
\addlinespace
AIDS & MPGX-CF & 100.0\% & $0.285 \pm 0.059$ & $1.002 \pm 0.040$ \\
AIDS & Greedy control & 100.0\% & $0.287 \pm 0.058$ & $1.021 \pm 0.065$ \\
AIDS & Random & 99.7\% & $0.285 \pm 0.059$ & $1.003 \pm 0.040$ \\
\addlinespace
COX2\_MD & MPGX-CF & 100.0\% & $0.025 \pm 0.005$ & $0.998 \pm 0.028$ \\
COX2\_MD & Greedy control & 100.0\% & $0.025 \pm 0.005$ & $1.018 \pm 0.059$ \\
COX2\_MD & Random & 100.0\% & $0.025 \pm 0.005$ & $0.998 \pm 0.027$ \\
\addlinespace
BBBP & MPGX-CF & 99.7\% & $0.277 \pm 0.052$ & $1.008 \pm 0.094$ \\
BBBP & Greedy control & 100.0\% & $0.286 \pm 0.052$ & $1.137 \pm 0.186$ \\
BBBP & Random & 98.9\% & $0.268 \pm 0.059$ & $0.998 \pm 0.084$ \\
\addlinespace
\bottomrule
\end{tabular}


==> submission_baseline_factual.tex <==
\begin{tabular}{lllcc}
\toprule
Dataset & Method & Success & Retained & Comp. \\
\midrule
MUTAG & MPGX-CF & 100.0\% & $0.105 \pm 0.131$ & $0.120 \pm 0.220$ \\
MUTAG & GNNExplainer & 100.0\% & $0.160 \pm 0.210$ & $0.103 \pm 0.213$ \\
MUTAG & PGExplainer & 100.0\% & $0.219 \pm 0.280$ & $0.112 \pm 0.243$ \\
MUTAG & CF$^2$ reimplementation & 96.8\% & $0.445 \pm 0.154$ & $0.519 \pm 0.355$ \\
MUTAG & Random & 100.0\% & $0.183 \pm 0.222$ & $0.114 \pm 0.220$ \\
\addlinespace
Mutagenicity & MPGX-CF & 100.0\% & $0.155 \pm 0.203$ & $0.142 \pm 0.241$ \\
Mutagenicity & GNNExplainer & 100.0\% & $0.209 \pm 0.262$ & $0.118 \pm 0.226$ \\
Mutagenicity & PGExplainer & 100.0\% & $0.266 \pm 0.331$ & $0.140 \pm 0.247$ \\
Mutagenicity & CF$^2$ reimplementation & 96.8\% & $0.579 \pm 0.153$ & $0.417 \pm 0.283$ \\
Mutagenicity & Random & 100.0\% & $0.229 \pm 0.281$ & $0.103 \pm 0.214$ \\
\addlinespace
AIDS & MPGX-CF & 100.0\% & $0.103 \pm 0.079$ & $0.019 \pm 0.113$ \\
AIDS & GNNExplainer & 100.0\% & $0.112 \pm 0.112$ & $0.018 \pm 0.109$ \\
AIDS & PGExplainer & 100.0\% & $0.111 \pm 0.115$ & $0.014 \pm 0.103$ \\
AIDS & CF$^2$ reimplementation & 61.7\% & $0.405 \pm 0.186$ & $0.094 \pm 0.212$ \\
AIDS & Random & 100.0\% & $0.113 \pm 0.118$ & $0.017 \pm 0.106$ \\
\addlinespace
COX2\_MD & MPGX-CF & 100.0\% & $0.092 \pm 0.218$ & $0.048 \pm 0.173$ \\
COX2\_MD & GNNExplainer & 100.0\% & $0.115 \pm 0.248$ & $0.057 \pm 0.178$ \\
COX2\_MD & PGExplainer & 100.0\% & $0.177 \pm 0.322$ & $0.072 \pm 0.206$ \\
COX2\_MD & CF$^2$ reimplementation & 56.5\% & $0.112 \pm 0.151$ & $0.139 \pm 0.264$ \\
COX2\_MD & Random & 100.0\% & $0.085 \pm 0.192$ & $0.031 \pm 0.130$ \\
\addlinespace
BBBP & MPGX-CF & 100.0\% & $0.086 \pm 0.093$ & $0.090 \pm 0.163$ \\
BBBP & GNNExplainer & 100.0\% & $0.145 \pm 0.169$ & $0.071 \pm 0.128$ \\
BBBP & PGExplainer & 100.0\% & $0.186 \pm 0.248$ & $0.072 \pm 0.141$ \\
BBBP & CF$^2$ reimplementation & 95.3\% & $0.542 \pm 0.122$ & $0.521 \pm 0.269$ \\
BBBP & Random & 100.0\% & $0.182 \pm 0.210$ & $0.067 \pm 0.132$ \\
\addlinespace
\bottomrule
\end{tabular}


==> submission_chemistry_fragment_analysis.tex <==
\begin{tabular}{lcccccc}
\toprule
View & Success & Steps & Atoms removed & Tanimoto & Retained $p_y$ ratio & Candidates \\
\midrule
Factual & 97.7\% & $1.71 \pm 0.70$ & $19.91 \pm 8.79$ & $0.10 \pm 0.11$ & $0.92 \pm 0.12$ & $56.98 \pm 59.75$ \\
Counterfactual & 27.4\% & $1.40 \pm 0.61$ & $3.22 \pm 2.66$ & $0.62 \pm 0.14$ & $0.56 \pm 0.15$ & $73.96 \pm 66.97$ \\
Exemplar & 96.4\% & $2.19 \pm 0.78$ & $6.63 \pm 2.60$ & $0.35 \pm 0.12$ & $1.00 \pm 0.14$ & $57.54 \pm 59.95$ \\
\bottomrule
\end{tabular}


==> submission_cross_perspective_overlap.tex <==
\begin{tabular}{lccc}
\toprule
Dataset & Factual--CF overlap & Factual--exemplar overlap & Contrast \\
\midrule
MUTAG & $0.095 \pm 0.187$ & $0.017 \pm 0.048$ & $0.078 \pm 0.177$ \\
Mutagenicity & $0.150 \pm 0.212$ & $0.036 \pm 0.065$ & $0.114 \pm 0.214$ \\
AIDS & $0.259 \pm 0.211$ & $0.075 \pm 0.083$ & $0.184 \pm 0.204$ \\
COX2\_MD & $0.014 \pm 0.029$ & $0.005 \pm 0.008$ & $0.009 \pm 0.030$ \\
BBBP & $0.177 \pm 0.210$ & $0.026 \pm 0.048$ & $0.151 \pm 0.199$ \\
\bottomrule
\end{tabular}


==> submission_model_calibration.tex <==
\begin{tabular}{llcccc}
\toprule
Dataset & Architecture & Brier & ECE & Log loss & Best epoch \\
\midrule
AIDS & GCN & $0.015 \pm 0.006$ & $0.023 \pm 0.007$ & $0.077 \pm 0.050$ & 37.8 \\
BBBP & GCN & $0.122 \pm 0.005$ & $0.094 \pm 0.010$ & $0.466 \pm 0.035$ & 10.3 \\
COX2\_MD & GCN & $0.285 \pm 0.065$ & $0.204 \pm 0.127$ & $0.865 \pm 0.382$ & 6.9 \\
MUTAG & GCN & $0.162 \pm 0.045$ & $0.204 \pm 0.046$ & $0.494 \pm 0.114$ & 51.2 \\
Mutagenicity & GCN & $0.153 \pm 0.012$ & $0.052 \pm 0.012$ & $0.494 \pm 0.053$ & 86.8 \\
\bottomrule
\end{tabular}


==> submission_model_performance.tex <==
\begin{tabular}{llcccc}
\toprule
Dataset & Architecture & Balanced accuracy & AUROC & AUPRC & F1 \\
\midrule
AIDS & GCN & $0.971 \pm 0.014$ & $0.985 \pm 0.015$ & $0.991 \pm 0.012$ & $0.989 \pm 0.005$ \\
BBBP & GCN & $0.698 \pm 0.014$ & $0.797 \pm 0.010$ & $0.942 \pm 0.008$ & $0.907 \pm 0.008$ \\
COX2\_MD$^{\dagger}$ & GCN & $0.519 \pm 0.069$ & $0.561 \pm 0.133$ & $0.586 \pm 0.099$ & $0.522 \pm 0.181$ \\
MUTAG & GCN & $0.688 \pm 0.160$ & $0.836 \pm 0.102$ & $0.929 \pm 0.043$ & $0.835 \pm 0.062$ \\
Mutagenicity & GCN & $0.781 \pm 0.024$ & $0.856 \pm 0.022$ & $0.819 \pm 0.029$ & $0.757 \pm 0.027$ \\
\bottomrule
\end{tabular}


==> submission_results_abstract_sentence.tex <==
On the five datasets, hard-constraint coverage ranged from 100.0\% for factual explanations, 4.8--67.6\% for counterfactuals, and 98.9--100.0\% for exemplars; conditional quality is reported only alongside these denominators.


==> submission_results_conclusion_sentence.tex <==
Empirically, the locked test run obtained 100.0\% factual, 4.8--67.6\% counterfactual, and 98.9--100.0\% exemplar coverage across datasets, demonstrating why discrete success and conditional quality must be reported separately.


==> submission_results_explanation_narrative.tex <==
Across datasets, hard factual coverage was 100.0\% and successful factuals retained 0.09--0.16 of input edges. Counterfactual flip coverage was 4.8--67.6\%; successful flips removed 2.59--4.68 edges on average, depending on the dataset. Exemplar preservation coverage was 98.9--100.0\%; successful exemplars edited 0.02--0.29 of edges while retaining 1.00--1.05 of the query-class confidence. These conditional ranges are interpreted only together with their coverage denominators.


==> submission_results_predictor_narrative.tex <==
Held-out GCN AUROC ranged from $0.561 \pm 0.133$ on COX2\_MD to $0.985 \pm 0.015$ on AIDS. The prespecified weak-predictor rule flagged COX2\_MD; its explanation results characterize that frozen model rather than application utility.


==> submission_structural_diagnostics.tex <==
\begin{tabular}{llccccccc}
\toprule
Dataset & View & Present & Removed & Removed frac. & $|\Delta p|$ & $\Delta$ betw. & $\Delta$ harmonic & Stability \\
\midrule
MUTAG & Factual & $1.98 \pm 2.71$ & $17.82 \pm 6.05$ & $0.90 \pm 0.13$ & $0.08 \pm 0.09$ & $0.22 \pm 0.04$ & $6.27 \pm 1.25$ & $0.25 \pm 0.35$ \\
MUTAG & Counterfactual & $17.33 \pm 5.22$ & $2.59 \pm 1.57$ & $0.13 \pm 0.07$ & $0.44 \pm 0.19$ & $0.12 \pm 0.05$ & $1.68 \pm 0.97$ & $0.74 \pm 0.29$ \\
MUTAG & Exemplar & $14.27 \pm 4.33$ & $5.52 \pm 1.75$ & $0.28 \pm 0.05$ & $0.08 \pm 0.08$ & $0.16 \pm 0.04$ & $3.33 \pm 0.78$ & $0.19 \pm 0.13$ \\
\addlinespace
Mutagenicity & Factual & $4.33 \pm 6.97$ & $26.44 \pm 16.25$ & $0.84 \pm 0.20$ & $0.12 \pm 0.10$ & $0.21 \pm 0.05$ & $7.92 \pm 2.50$ & $0.42 \pm 0.38$ \\
Mutagenicity & Counterfactual & $26.13 \pm 15.08$ & $2.85 \pm 1.91$ & $0.11 \pm 0.07$ & $0.31 \pm 0.16$ & $0.10 \pm 0.06$ & $2.44 \pm 1.28$ & $0.74 \pm 0.30$ \\
Mutagenicity & Exemplar & $24.11 \pm 15.79$ & $6.69 \pm 1.83$ & $0.25 \pm 0.07$ & $0.08 \pm 0.06$ & $0.16 \pm 0.06$ & $4.33 \pm 0.98$ & $0.17 \pm 0.13$ \\
\addlinespace
AIDS & Factual & $1.24 \pm 1.35$ & $14.96 \pm 15.03$ & $0.90 \pm 0.08$ & $0.02 \pm 0.05$ & $0.27 \pm 0.07$ & $5.13 \pm 1.88$ & $0.06 \pm 0.19$ \\
AIDS & Counterfactual & $14.45 \pm 4.53$ & $3.48 \pm 2.10$ & $0.19 \pm 0.09$ & $0.42 \pm 0.16$ & $0.17 \pm 0.07$ & $2.57 \pm 1.24$ & $0.94 \pm 0.14$ \\
AIDS & Exemplar & $12.23 \pm 13.45$ & $3.97 \pm 1.98$ & $0.29 \pm 0.06$ & $0.01 \pm 0.03$ & $0.20 \pm 0.07$ & $2.71 \pm 0.87$ & $0.24 \pm 0.10$ \\
\addlinespace
COX2\_MD & Factual & $30.99 \pm 75.25$ & $304.14 \pm 96.02$ & $0.91 \pm 0.22$ & $0.07 \pm 0.07$ & $0.01 \pm 0.03$ & $21.93 \pm 6.98$ & $0.08 \pm 0.22$ \\
COX2\_MD & Counterfactual & $313.68 \pm 51.22$ & $4.68 \pm 2.33$ & $0.02 \pm 0.01$ & $0.10 \pm 0.11$ & $0.00 \pm 0.00$ & $0.44 \pm 0.19$ & $0.31 \pm 0.28$ \\
COX2\_MD & Exemplar & $327.15 \pm 65.22$ & $7.97 \pm 0.34$ & $0.02 \pm 0.00$ & $0.01 \pm 0.02$ & $0.00 \pm 0.00$ & $0.47 \pm 0.04$ & $0.02 \pm 0.01$ \\
\addlinespace
BBBP & Factual & $2.19 \pm 2.35$ & $25.70 \pm 9.64$ & $0.91 \pm 0.09$ & $0.08 \pm 0.07$ & $0.23 \pm 0.03$ & $7.30 \pm 1.31$ & $0.38 \pm 0.35$ \\
BBBP & Counterfactual & $23.63 \pm 9.02$ & $3.65 \pm 2.24$ & $0.14 \pm 0.08$ & $0.38 \pm 0.15$ & $0.14 \pm 0.06$ & $2.61 \pm 1.22$ & $0.86 \pm 0.21$ \\
BBBP & Exemplar & $20.54 \pm 8.85$ & $7.35 \pm 1.19$ & $0.28 \pm 0.05$ & $0.05 \pm 0.05$ & $0.19 \pm 0.04$ & $4.06 \pm 0.56$ & $0.16 \pm 0.06$ \\
\addlinespace
\bottomrule
\end{tabular}

